Genome Variant Calling with a Deep Averaging Network

Variant calling, the problem of estimating whether a position in a DNA sequence differs from a reference sequence, given noisy, redundant, overlapping short sequences that cover that position, is fundamental to genomics. We propose a deep averaging network designed specifically for variant calling. Our model takes into account the independence of each short input read sequence by transforming individual reads through a series of convolutional layers, limiting the communication between individual reads to averaging and concatenating operations. Training and testing on the precisionFDA Truth Challenge (pFDA), we match state of the art overall 99.89 F1 score. Genome datasets exhibit extreme skew between easy examples and those on the decision boundary. We take advantage of this property to converge models at 5x the speed of standard epoch-based training by skipping easy examples during training. To facilitate future work, we release our code, trained models and pre-processed public domain datasets.

==> analysis.tex <==
\section{Analysis}
Our model out-performed DeepVariant on the pFDA Truth Challenge when trained on the HG001 dataset only. We were about as accurate on SNPs and much more accurate on Indels, although not quite as accurate on Indels as the overall Indels winner "dgrover-GATK." %Had we submitted these predictions to the challenge, we would have had the best overall F1 of all of the competitors, and won prizes for best Indel precision, and best SNPs F1.

Since the FDA Challenge, DeepVariant has significantly improved the accuracy of their model, primarily by training on large amounts of additional genomic data. These datasets are mentioned in the DeepVariant release notes, but not all of the data is uniquely identified, or publicly available. \footnote{\url{https://github.com/google/deepvariant/releases}}

Trained with additional data we show that our model also improves accuracy on the pFDA test data. Future work involves investigating the accuracy of this model when trained on larger and more modern datasets.


==> future.tex <==
\section{Things that did not work}
\subsection{Deeper networks and training stability}
We present results for a network with seven convolutional layers. We were able to train deeper networks with eight, nine or ten convolutional layers. However despite higher parameter counts, these did not converge to better training or test losses, and some exhibited numerical instability. 

As previously noted, we trained our networks with focal loss of 0.001 for enhanced stability. Deeper networks, and especially those with intermediate layer losses, were only stable with focal loss values of 0.01 or higher, which seems to contribute negatively to test performance. It is possible that deeper networks require more care in initialization and learning rate schedule. Although these deeper networks often only diverged after several epochs of training, suggesting that learning rate was not the problem. The seven layer networks reported in the results never diverged with a focal loss of 0.001 or higher, over many episodes of training. 

\subsection{Lower trainable parameter count}
DeepVariant uses the InceptionNet which has reduced the paramater count for a SOTA image classification network to 26 million trainable parameters {Cite inception V3}. Our best network uses 76 million parameters, although most of these are contained in the single layer going into the fully connected network.

We concatenate the outputs of the mean pool, the max pool, and the highway layers. Together that comprises 70,000 feature connecting to a 1,024 feature layer. We made several attempts to reduce the complexity of this layer, but each led to a noticeable drop in accuracy [see table]. 
Removing the max pool layer 
Reducing the number of channels going into the mean and max pool from 128, to 64 and 32
Averaging the highway outputs, instead of concatenating from every layer.

\subsection{Remove the highway layers}
We show it is possible to still converge reasonably good accuracy on the pFDA problem with a much smaller 17 million parameter network, but not without a noticeable drop in accuracy. Perhaps for some problems this tradeoff is worth it.

It is likely that there is a different dimension reduction technique that would be more effective toward this task, than the ones we tried.

\subsection{Data augmentation}
Given that variant calling is mostly a counting problem -- how many reads agree with the variant, and what is the quality of those reads -- it seems likely that problem-specific data augmentation could help converge a more generalizable network. Indeed, data augmentation through down-sampling a BAM to create a lower coverage dataset is used by DeepVariant, and the pFDA dataset is created by down-sampling a larger Illumina HiSeq dataset down to 50x coverage. 

However, we did not observe noticeable gains from dynamically down-sampling reads coverage during training.

Moreover, we did not observe improvement from directionally down-sampling reads either matching or not matching the variant, and imposing a ranking penalty on those results. 

It seems at the moment, that the best way to improve a deep variant calling model is through more high quality training data, perhaps down-sampled to simulate lower read coverage. In the longer term, it seems likely that a more sophisticated method of data augmentation would be useful for simulating sequencing machine errors, as well as errors in alignment and other upstream processes. 

\subsection{Train only on difficult regions} %[Scripps]
Given our success skipping 85\% of all easy locations after the first epoch, we tried importing only the non-easy locations for 10x genome datasets [from Scripps, what’s it called?]. Specifically, we collected all “not well classified” locations after two epochs of training, on the precisionFDA training set only and for each of the 10x datasets, imported
\begin{itemize}
    \item All variant candidates for 54,000 locations, identified as non-easy from the pFDA training set \footnote{precisionFDA and Scripps are all HG001, but even across human genomes, difficult locations are occurrence of Indel mutations are highly correlated between individuals}
    \item An equal number of random variant candidates from the same genome dataset
\end{itemize}
This dataset was very appealing, because instead of importing 6-12 million candidates per dataset, we could import 100,000 examples, focusing on long Indels and other difficult locations of the human genome. 

However, this did not lead to improved test accuracies, and actually generalized worse than just training on the pFDA training set, despite adding 3x full Scripps datasets significantly improving generalization.

There likely is a middle ground between these two approaches. If so, it would be extremely helpful to reduce training dataset size, when training on a growing collection of genome datasets.   

\subsection{NovaSeq without re-alignment}
The precisionFDA dataset and all of the Scripps datasets are sequence on Illumina HiSeq machines. We found a public Illumina NovaSeq dataset [Illumina website] for HG001, and ran a chromosome holdout experiment -- since it is well documented that DeepVariant is never trained on HG001, Chromosome 10. 

Our results (99.81 F1) were substantially worse than DeepVariant v0.7 (99.94 F1) as well as the non deep learning Senteion tool (99.88 F1). However, a deeper analysis of the errors showed that many (how many?) of the false negatives of our predictions were not even variant candidates for GenoVarONN, while Senteion and DeepVariant were able to predict these mutations correctly. This goes to show the complexity of the variant calling problem. Starting with a globally aligned BAM file may be sufficient for pFDA, but local re-alignment for Indels becomes critical to variant calling performance for other datasets, both for training and testing. It is not simple to compare variant calling neural networks, without taking upstream data processing into account. 

